Hierarchical Generation of Human-Object Interactions with Diffusion Probabilistic Models

This paper presents a novel approach to generating the 3D motion of a human interacting with a target object, with a focus on solving the challenge of synthesizing long-range and diverse motions, which could not be fulfilled by existing auto-regressive models or path planning-based methods. We propose a hierarchical generation framework to solve this challenge. Specifically, our framework first generates a set of milestones and then synthesizes the motion along them. Therefore, the long-range motion generation could be reduced to synthesizing several short motion sequences guided by milestones. The experiments on the NSM, COUCH, and SAMP datasets show that our approach outperforms previous methods by a large margin in both quality and diversity. The source code is available on our project page https://zju3dv.github.io/hghoi.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/05_milestone.tex <==
\begin{table}[tb]
\centering
\scriptsize{
\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{1.3}
    \setlength\tabcolsep{2pt}
        \begin{tabular}{ccc|ccccccc}
        \hline
        GP & KP & KT & FD$\downarrow$ & $\text{R-APD}_{M}\uparrow$ & $\text{R-APD}_{P}\uparrow$ & $\text{R-APD}_{T}\uparrow$ & $\text{F-APD}_{M}\uparrow$ & $\text{F-APD}_{P}\uparrow$ & $\text{F-APD}_{T}\uparrow$ \\
        \hline
        & \checkmark & \checkmark & 31.07 & 3.21 & 2.46 & 85.21 & 2.55 & 0.75 & 61.52 \\
        \checkmark & & \checkmark & 25.14 & 4.01 & 3.78 & 85.69 & 3.74 & 3.06 & 76.64\\
        \checkmark&  &  &27.87 & 3.62 & 3.01 & \textbf{127.94} & 3.44 & 2.41 & \textbf{108.63} \\
        \checkmark & \checkmark & \checkmark & \textbf{22.29} & \textbf{4.17} & \textbf{4.52} & 91.38 & \textbf{4.01} & \textbf{4.41} & 83.41 \\
      \hline
    \end{tabular}
    }
}
\caption{\textbf{Ablation of milestone generation.} GP: goal pose generation. KP: milestone pose generation. KT: milestone trajectory generation.} 
\label{tab:milestone}
% \vspace{-2ex}
\end{table}
